Using Deep Q-learning To Prolong the Lifetime of Correlated Internet of Things Devices

Battery-powered sensors deployed in the Internet of Things (IoT) require energy-efficient solutions to prolong their lifetime. When these sensors observe a physical phenomenon distributed in space and evolving in time, the collected observations are expected to be correlated. We take advantage of the exhibited correlation and propose an updating mechanism that employs deep Q-learning. Our mechanism is capable of determining the frequency with which sensors should transmit their updates while taking into the consideration an ever-changing environment. We evaluate our solution using observations obtained in a real deployment, and show that our proposed mechanism is capable of significantly extending battery-powered sensors' lifetime without compromising the accuracy of the observations provided to the IoT service.

==> section_bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{male-silhouette}}]{Jernej Hribar}
currently is a PhD student at the
CONNECT (formerly CTVR) Telecommunications Research Centre at Trinity
College Dublin (Ireland).
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Nick_Kaminski}}]{Nicholas Kaminski}
 currently is a Research Fellow at the
CONNECT (formerly CTVR) Telecommunications Research Centre at Trinity
College Dublin (Ireland).  He conducts research focused on extending
the bounds of wireless technology by deploying targeted intelligence
to act in harmony with flexible radio systems.  He advances
distributed radio intelligence through experimentation-based research
and is co-principal investigator on several European projects that
create and develop experimentation platforms and services for an open
infrastructure. Dr. Kaminski received his master‘s degree in
Electrical Engineering in 2012 and his Ph.D. in 2014 from Virginia
Tech, USA. During this time he was funded as a Bradley Fellow at the
Bradley Department of Electrical and Computer Engineering at Virginia
Tech. He is a co-inventor on a preliminary patent application for his
work extending the utility of cognitive radios.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{johann_marquez-barja-April2015}}]{Johann M. Marquez-Barja}
is a Research Fellow at the CONNECT - Networks of the Future - Research Centre (formerly CTVR) at Trinity College Dublin (Ireland). His main research areas of interest are wireless/small cells architectures, mobility and optical/wireless integration. Also, he is interested on vehicular networks, vertical handover techniques and smart cities. Due to his lecturing activities, he is now applying his research outcome to education through technology enhanced learning techniques. He has studied in USA, Bolivia, Cuba and Spain. He holds a Systems Engineering Degree (graduated with honors), a MSc. on Telematics, a MsC on Computer Architecture and a PhD on Architecture and Technology of Computer Systems issued by the Universitat Politecnica de Valencia (Spain) [graduated with honors cum laude, as well]. On 2004 he received a personal grant from the EU under the Alban Programme to purse the PhD degree. Dr. Marquez-Barja is serving as Editor and Guest Editor for a number of International Journals, as well as being part of several organizing and technical programme committees at different worldwide conferences/congresses. At Trinity College Dublin he is also lecturing wireless networks and communications systems.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{LuizDaSilva_cartoon_2013}}]{Luiz A. DaSilva}
is the Professor of Telecommunications at Trinity College Dublin. He is also a Professor in the Bradley Department of Electrical and Computer
Engineering at Virginia Tech, USA. His research focuses on distributed and adaptive resource management in wireless
networks, and in particular wireless resource sharing, dynamic spectrum access, and the application of game theory to
wireless networks. Prof. DaSilva is currently a principal investigator on research projects funded by the National Science
Foundation in the United States, the Science Foundation Ireland, and the European Commission under Horizon 2020 and Framework
Programme 7. He is a co-principal investigator of CONNECT, the Telecommunications Research Centre in Ireland.
\end{IEEEbiography}
